Z3-Noodler: An Automata-based String Solver (Technical Report)

Z3-Noodler is a fork of Z3 that replaces its string theory solver with a custom solver implementing the recently introduced stabilization-based algorithm for solving word equations with regular constraints. An extensive experimental evaluation shows that Z3-Noodler is a fully-fledged solver that can compete with state-of-the-art solvers, surpassing them by far on many benchmarks. Moreover, it is often complementary to other solvers, making it a suitable choice as a candidate to a solver portfolio.

==> figs/table_pyex.tex <==
\newcolumntype{g}{>{\columncolor{gray!30}}r}
\newcolumntype{f}{>{\columncolor{gray!30}}l}
\newcolumntype{h}{>{\columncolor{gray!30}}c}
\newcommand{\ping}[0]{\bf}
\begin{tabular}{lgg}
\toprule
& \multicolumn{2}{h}{\pyex}\\
& \multicolumn{1}{h}{avg} & \multicolumn{1}{h}{std}\\
\midrule
\rowcolor{GreenYellow}
\ziiinoodler & 3.40 & 12.58 \\
\cvcv & 0.32 & 2.59 \\
\ziii & 2.77 & 10.54 \\
\ziiistriv & 1.45 & 6.43 \\
\ostrich & 54.97 & 78.76 \\
\ziiistriiire & 0.66 & 4.21 \\
\ziiinoodleroopsla & 2.98 & 10.41 \\
\end{tabular}

